Experimentation Platforms Meet Reinforcement Learning: Bayesian Sequential Decision-Making for Continuous Monitoring

With the growing needs of online A/B testing to support the innovation in industry, the opportunity cost of running an experiment becomes non-negligible. Therefore, there is an increasing demand for an efficient continuous monitoring service that allows early stopping when appropriate. Classic statistical methods focus on hypothesis testing and are mostly developed for traditional high-stake problems such as clinical trials, while experiments at online service companies typically have very different features and focuses. Motivated by the real needs, in this paper, we introduce a novel framework that we developed in Amazon to maximize customer experience and control opportunity cost. We formulate the problem as a Bayesian optimal sequential decision making problem that has a unified utility function. We discuss extensively practical design choices and considerations. We further introduce how to solve the optimal decision rule via Reinforcement Learning and scale the solution. We show the effectiveness of this novel approach compared with existing methods via a large-scale meta-analysis on experiments in Amazon.

==> 5_Literature.tex <==

\section{Literature Review (In Progress)}
\subsection{Dynamic Programming/RL for SDoE}
The classic SDoE problem typically focuses on maximizing the information gain. 
We first focus on a line of research on Bayesian SDoE. 
Consider a regression model $y_t = f(x_t; \theta) + \epsilon_t$. 
Our goal is to sequentially select $x_t$ (actions) so as to collect observations $y_t$ to accurately estimate $\theta$ (or predict something). 
In the Bayesian framework, this information gain is typically characterized by the mutual information, which then defines the reward. 

The problem is natural to be formulated as a SDM (or so-called DP) problem. 
The main challenges lies in how to solve this optimization problem, especially with continuous spaces and non-Gaussian (or even no-closed-form) distributions. 
A naive backwards induction (i.e., DP; RL for discrete space) solution has been shown as not computationally feasible \citep{muller2007simulation}, as in our previous numerical experiments. 
RL techniques such as  approximate DP (value-based RL) \citep{huan2016sequential} and 
policy gradient (policy-based RL \citep{shen2021bayesian} are latter applied to obtain an approximate solution. 
This problem is recently extended to even more challenging cases, where explicit model is not available but sampling from the distribution is feasible \citep{ivanova2021implicit, foster2021deep}. 


% Model-based
% equal to how the model family is known
% maximization the information gain
% different but can learn some 


% Overall, the papers above are about how to appropriately frame the problem as an RL task and apply SOTA algorithm to solve. 
% Our project 

% \hl{Our difference! (not , but the overall cost; early stopping; two samples and ATE estimation; discrete action space)}

\subsection{AVI and Sequential Testing}

% \hl{Other topics reviewed in those papers}




% The observed data consists of $n$ i.i.d. trajectories, and can be summarized as $\{(S_{i,t},A_{i,t},R_{i,t},S_{i,t+1})\}_{0\le t<T,1\le i\le n}$. 


==> 6_closed_form.tex <==

\section{Closed-form solution under the Normal-Normal model}
\begin{equation}
R_t =
\begin{cases}
     -c + \delta \times N_{1:t, Tr} &\text{when}  \;\; A_t = 0 \; \text{and} \; I_t = 0, %\text{(Not terminated \& keep running)} 
     \\
     \begin{aligned}
     \Mean_{\vthe \sim \rho(\vthe)}\big[ & \delta \mid \mathcal{H}_t \big] \bigg(\sum_{g}N_{1:T, g}\bigg) \\
     & \times (H + T - t) -c_h,
     \end{aligned} &\text{when} \; A_t = 1 \; \text{and} \;\; I_t = 0, 
     %\text{(Not terminated \& recommend launch)} 
    
     \\
     0, & \text{when} \;\;A_t = 2  \; \text{and} \; I_t = 0, 
     %\text{(Not terminated \& recommend no launch)} 
     \\
     0, & \text{when}\;\;I_t = 1, 
     %\text{(Already terminated)}.
     \end{cases}
     \label{eq:reward}
\end{equation}


$V^*_T(S_T) = 
\max \Bigg(
     \Mean_{\vthe \sim \rho(\vthe)}\big[  \delta \mid \mathcal{H}_T \big] \bigg(\sum_{g}N_{1:T, g}\bigg)
    \times H -c_h, 0
\Bigg
) I(I_T = 0)$


\begin{align*}
Q^*_t(S_t, a) 
&= r(S_t, a) + \Mean V^*_{t+1}(S_{t+1})\\
&= I(I_t = 0, a = 0) \times 
\Big[ 
 -c + \delta \times N_{1:t, Tr} 
 + \Mean V^*_{t+1}(S_{t+1})
\Big]\\
&+ 
I(I_t = 0, a = 1) \times 
\Big[ 
\Mean_{\vthe \sim \rho(\vthe)}\big[  \delta \mid \mathcal{H}_t \big] \bigg(\sum_{g}N_{1:T, g}\bigg) 
\times (H + T - t) -c_h
\Big]\\
V^*_t(S_t) &= \argmax_a Q^*_t(S_t, a) 
\end{align*}

Recall that our model is 


\begin{align*}
%  &\bar{W}_{l, *} | \mu_{*} \sim N \bigg( \frac{\mu_{*} \sum_{t = 1}^{l}N_{t, *}(l -t + 1)}{\sum_{t = 1}^l N_{t, *}}, \frac{\sigma_{*}^2}{(\sum_{t = 1}^l N_{t, *} )^2}  \sum_{t = 1}^{l} N_{t, *} (l- t + 1)
%  \bigg), \\
&\mu_{*}|  \bar{W}_{l, *}  
\sim N\bigg(\bigg( \frac{1}{\tau_{*}^2} + \frac{a_{*}(l)^2}{\sigma_{*}^2 b_{*}(l)} \bigg)^{-1}    \bigg( \frac{\mu_{0*}}{\tau_{*}^2} + \frac{a_{*}(l) \bar{W}_{l, *}}{\sigma_{*}^2 b_{*}(l)}\bigg)    ,\bigg( \frac{1}{\tau_{*}^2} + \frac{a_{*}(l)^2}{\sigma_{*}^2 b_{*}(l)} \bigg)^{-1}\bigg), \\
&\bar{W}_{l+1, *} | \mu_{*}, \bar{W}_{l, *} \sim N \bigg(
\frac{\bar{W}_{l, *}  N_{1:l, *} + \mu_{*}  N_{1:l+1, *} }{N_{1:l+1, *}}, \frac{1}{N_{1:l+1, *}} \sigma^2_{*}
\bigg). 
\end{align*}


\begin{align*}
&\Mean\big[\mu_{*}|  \bar{W}_{l, *} \big]
= \bigg( \frac{1}{\tau_{*}^2} + \frac{a_{*}(l)^2}{\sigma_{*}^2 b_{*}(l)} \bigg)^{-1}    \bigg( \frac{\mu_{0*}}{\tau_{*}^2} + \frac{a_{*}(l) \bar{W}_{l, *}}{\sigma_{*}^2 b_{*}(l)}\bigg)\\
&= A_{*,l} + B_{*,l} \bar{W}_{l, *}
\end{align*}

So $\Mean_{\vthe \sim \rho(\vthe)}\big[ \delta \mid \mathcal{H}_t \big]$ is a linear transformation of $(\bar{W}_{l, T}, \bar{W}_{l, C})$. 

So does the mean of $\bar{W}_{l+1, *}$. (but is it determined by the mean??

\red{To be completed. }

==> Mis/packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{textcomp}
\usepackage{enumitem}
\usepackage{datetime2}
\usepackage{multirow}
\usepackage[font=small,labelfont=bf]{caption}
\doublespacing
\usepackage{subcaption}

\usepackage{xcolor}



\usepackage{lineno}
\linenumbers


% from cjhebrew.sty (with scaling added)
\DeclareFontFamily{U}{cjheb}{}
\DeclareFontShape{U}{cjheb}{m}{n}{%
  <-11> s*[1.2] cjhblsm
  <11-> s*[1.2] cjhbltx
}{}
\newcommand{\cjhebfamily}{\fontencoding{U}\fontfamily{cjheb}\selectfont}
\DeclareTextFontCommand{\textcjheb}{\cjhebfamily}

% provide the commands in case amssymb is not loaded
\providecommand{\beth}{}
\providecommand{\gimel}{}
\providecommand{\daleth}{}
% renew the commands
\newcommand{\mathhebrew}[1]{\text{\cjhebfamily#1}}
\renewcommand{\aleph}{\mathhebrew{\char'047}}
\renewcommand{\beth}{\mathhebrew{\char'142}}
\renewcommand{\gimel}{\mathhebrew{\char'147}}
\renewcommand{\daleth}{\mathhebrew{\char'144}}

% \usepackage{unicode-math}
% \usepackage{libertine}
% \setmathfont[range={\beth,\gimel,\daleth,\aleph}]{Linux Libertine O}   

